Crowd-sensing Enhanced Parking Patrol using Trajectories of Sharing Bikes

Illegal vehicle parking is a common urban problem faced by major cities in the world, as it incurs traffic jams, which lead to air pollution and traffic accidents. The government highly relies on active human efforts to detect illegal parking events. However, such an approach is extremely ineffective to cover a large city since the police have to patrol over the entire city roads. The massive and high-quality sharing bike trajectories from Mobike offer us a unique opportunity to design a ubiquitous illegal parking detection approach, as most of the illegal parking events happen at curbsides and have significant impact on the bike users. The detection result can guide the patrol schedule, i.e. send the patrol policemen to the region with higher illegal parking risks, and further improve the patrol efficiency. Inspired by this idea, three main components are employed in the proposed framework: 1)~{\em trajectory pre-processing}, which filters outlier GPS points, performs map-matching, and builds trajectory indexes; 2)~{\em illegal parking detection}, which models the normal trajectories, extracts features from the evaluation trajectories, and utilizes a distribution test-based method to discover the illegal parking events; and 3)~{\em patrol scheduling}, which leverages the detection result as reference context, and models the scheduling task as a multi-agent reinforcement learning problem to guide the patrol police. Finally, extensive experiments are presented to validate the effectiveness of illegal parking detection, as well as the improvement of patrol efficiency.

==> exp-bak.tex <==
\section{Experiments}~\label{sec:exp}

In this section, we conduct extensive experiments to evaluate the effectiveness and efficiency of our system. We first describe the real dataset used in the paper. Then, we give experiment results to select the proper threshold $\alpha$ used in the KS-test. Then, effectiveness comparisons between different baseline solutions are provided. After that, we test the efficiency performance of our system based on different sizes of Storm clusters. Finally, a set of real case studies are presented to demonstrate the effectiveness of our solution.

% https://scholar.google.com/scholar?hl=en&as_sdt=0%2C9&q=imbalanced+data+neural+network&btnG=&oq=imbalanced+data+neural
\subsection{Datasets}

  \sstitle{Road Networks} Road network of Beijing, China is from Open Street Map~\footnote{\url{https://www.openstreetmap.org/}} with $377,559$ nodes and $501,462$ edges.

  \sstitle{Mobike Trajectories}  Each Mobike trajectory contains a bike ID, a user ID, a temporal range of the trajectory, a pair of start/end locations, and a sequence of intermediate GPS points. 
  
The dataset used in the paper is the full Mobike trajectory data in the City of Beijing, with the time span of 08/01/2017 - 2/08/2018, the spatial distribution is shown in Figure~\ref{fig:opportunity}a~\footnote{The detailed statistics of the trajectory dataset are not disclosed in the paper, due to the request from Mobike.}.

  \sstitle{Ground Truth Labels} We collected a set of ground truth labels for illegal parking events in both Chaoyang and Haidian District, in Beijing. Each record contains a road ID, a timestamp, a photo, and a label to indicate the presence of illegal parking events.

The dataset covers 32 roads, and spans over $18$ days (12/26/2017 - 12/30/2017 in Haidian, and 01/12/2018 - 02/09/2018 in Chaoyang). Overall, the $454$ ground truth labels are collected, with 159 records labelled as positive (i.e., with illegal parking events).

\subsection{Effectiveness Evaluation}~\label{sec:exp:effectiveness}

In this subsection, we evaluate the effectiveness of the proposed detection model. We first introduce the process to select the most effective threshold for KS-test. Then, we compare our algorithm with three baseline methods. Finally, we study the effectiveness of detection model with different numbers of trajectories.

\sstitle{Threshold Selection} In our implementation, we tried all possible threshold probability $\alpha$ in our KS-test from 0 to 1 with the step size of 0.01. To determine the most effective threshold, we test the detection result with the ground truth labels. A F1 score is calculated to reflect the effectiveness of different threshold values. In detail, we count the numbers of True Positives $N_{TP}$ (i.e., correct identification of positive labels), False Positives $N_{FP}$ (i.e., incorrect identification of positive labels), and False Negatives $N_{FN}$ (i.e., incorrect identification of negative labels) to calculate F1-score: 

    \begin{equation}\label{eqn:f1}
      \begin{split}
        P &= N_{TP}/(N_{TP}+N_{FP}),
        \\
        R &= N_{TP}/(N_{TP}+N_{FN}),
        \\
        F_1 &= 2PR/(P+R).
      \end{split}
    \end{equation} 

Figure~\ref{fig:exp:exp}a presents the F1 scores with the corresponding \textit{precision} $P$ and \textit{recall} $R$ with respect of different threshold values $\alpha$: 1)~when $\alpha$ is close to zero, all the test data are labelled as negative, so both precision and recall are 0; 2)~with the increase of $\alpha$, more and more instances are labeled as positive, and we identify that $\alpha=0.71$ is the best selection as F1-score reaches the maximum of $0.73$. As a result, we use $\alpha=0.71$ as the threshold in our system.



\begin{figure}[t]
  \begin{center}
  \includegraphics[width=3.4in]{./Figures/exp.pdf}
    \caption{Effectiveness \& Efficiency Experiments.}
  \label{fig:exp:exp}
  \end{center}
  \vspace{-30pt}
\end{figure}

%Note that although \textit{precision} can reach almost $0.80$ when $\alpha$ is set to 0.35, the \textit{recall} is below $0.4$ and loses the ability to be ubiquitous.

%
% Based on our algorithm introduced in Section~\ref{sec:detection:kstest}, we take mainly three steps to select the optimal threshold $\alpha$: 1)~Test Result Computation. 2)~Evaluation. Given the ground truth data collected, we evaluate each of the test result. F1-score, which has been the optimizaiton target in many existing works (e.g. \cite{tfHXW15,tfFIS08,tfLEN14}), is adopted as evaluation metric here.


 %    In this paper, we search all threshold space, i.e. from $0$ to $1$, with step $0.01$. We compare all the 101 F1-scores and as a result, we find \textbf{$\alpha=0.28$} the best threshold with \textbf{$F_1=0.75$.}

\sstitle{Compare with Baselines} To achieve a comprehensive comparison with different baseline approaches, we plot the Receiver operating characteristic (ROC curves) for each method. ROC curve illustrates the diagnostic ability of a binary classifier, which plots the true positive rate $TPrate=N_{TP}/(N_{TP}+N_{FN})$ and the false positive rate $FPrate=N_{FP}/(N_{FP}+N_{TN})$ of a model with different parameter settings (i.e., threshold $\alpha$). A method is better, if its AUC (Area Under Curve) is larger.

%  plot the 
%    To extensively compare our algorithm with other baseline methods, we calculate the areas under the ROC curve (AUC) of them. AUC serves as a single value mesurement for classifer performance and is invariant to the parameter change\cite{tfBAP97}. It has been widely used in comparing machine learning models (e.g. \cite{tfJWF10,tfTLM11}). Given TP rate $TPrate=N_{TP}/(N_{TP}+N_{FN})$ and FP rate $FPrate=N_{FP}/(N_{FP}+N_{TN})$ of a model, ROC curve is plotted as the parameter of the model varies. Then AUC is calculated as the trapezoidal integration of ROC curve.

In this experiment, we compare our deployed solution (i.e., \textit{Nt+Dir+T}) with three baseline methods:

{$\bullet$} \textbf{Naive.} It uses the shape of the road segment directly as baseline model, i.e., the shift distribution is set as a Gaussian Distribution with zero mean and $2\sigma$ value is set as $10$ meters. {\em Average shift extraction} is used for processing the evaluation trajectories.

{$\bullet$} \textbf{Nt.} It uses the aggregated night time trajectories to build the baseline model. The features are extracted based on {\em average shift extraction} method.

{$\bullet$} \textbf{Nt+Dir.} In addition to use the night time trajectories as the baseline mode, it also filters the reversed trajectories in each road segment. The trajectory features are extracted based on {\em average shift extraction} method.

{$\bullet$} \textbf{Nt+Dir+T.} It uses the same baseline model as {\em Nt.+Dir}, while {\em top shift extraction} method is employed to extract the features of evaluation trajectories.
 
Figure~\ref{fig:exp:exp}b presents the ROC curves of the 4 baseline methods by varying the threshold $\alpha$ of KS-test. In the measurement of AUC, our deployed method, i.e.,~\textit{Nt+Dir+T} outperforms other three methods significantly, since it considers both directional information and top shift features. The method considering the directional information and removing all the reverse trajectories is much better than the others, which demonstrates the necessity of reverse trajectory removal in the {\em pre-processing} component. Also in the \textit{Naive}, the TP rate is always smaller than FP rate, which implies the inaccuracy of GPS position cannot be neglected.

    
\sstitle{Different Trajectory Numbers} We study the influence of the detection effectiveness with different numbers of trajectories in the evaluation trajectory feature extraction step. In this experiment, we only choose a portion of labelled road segments with the number of trajectories over 50 in one hour time range, and down samples the dataset randomly to mimic the road with different numbers of trajectories from 10 to 50.

Figure~\ref{fig:exp:exp}c illustrates the ROC curves of our deployed method with different numbers of trajectories used for detection. From the figure we can see that the detection performance increases, when more trajectories can be used. Moreover, when the number of trajectories can be used for detection is less than 20, the detection accuracy is unstable. It confirms the necessity of using the crowd-wisdom to overcome the impacts from skewed individual riding behaviors and the limited GPS accuracy. Finally, the performance of detection model increases slightly when the number of trajectories is over 30. It shows that as long as it has enough number of trajectories (e.g., 30) in an hour on a road segment, our method can provide a relatively accurate detection result.

\subsection{Efficiency Evaluation}

The system response time is also tested to show the efficiency of our cloud-based deployment. The experiments are performed in Haidian District, which contains 10\% of the total trajectories in Beijing. We tested the different numbers of requests (i.e., to evaluate 1, 2, 4, and 8 hours of trajectories in the area, the evaluation requests with more than one hour perform the one-hour detection multiple times) with different numbers of worker nodes in Storm.

Figure~\ref{fig:exp:exp}d gives the results of system response time with different settings. We have the following two observations: 1)~the execution time decreases significantly by nearly $50\%$ when adding the number of workers from 1 to 2 and 2 to 4, since the detection tasks are distributed among the worker nodes; and 2)~when the number of workers increases further to 16, the performance gain is much less. This is due to the communication overhead of worker nodes. In terms of different sizes of trajectory data, the response time difference is relatively minor, as the MongoDB cluster provides an efficient trajectory data retrieval interface.

%\sstitle{Different query size} It is easy to find that our system is less sensitive to the query size, e.g. execution time of 8 hours' query is about 1.25 times of 1 hour's. The result shows that given 16 workers, our Storm-based system is efficient to update detection result in nearly one minute for hours of query size.



\subsection{Case Studies}

We conduct real world case studies to validate the effectiveness of our detection model. Moreover, we get some interesting observations by exploring the temporal variance of KS statistics.

\sstitle{Overall Rankings} To reflect the severity of the illegal parking events on the roads, we rank them based on the daily average hours with illegal parking events. To validate the correctness of our result, we conduct an on-site case study in the area of Figure~\ref{fig:exp:overallcase}). The area marked with the red dotted lines suffers from sever illegal parking events, based on our calculations. The reason becomes clear, when we got there. It is a very crowded area, with a lot of foreign embassies and high-end restaurants, but with very limited parking spaces. As a result, many people have to leave their cars in the bike lanes or on the pedestrian crossing  (as demonstrated in the left portion of the figure). On the other side, at the east side of the East 3rd ring road, the overall rankings of the green road segments are very low. It is because the POI distribution there is very sparse, with only two large hotels, and the Agriculture Exhibition Center. All of these places are facilitated with very large parking lots. As a result, as shown in the right portion of the figure, the road are clear without any illegal parking events.
  
%  
%  Figure~\ref{fig:exp:case}a shows the ranking results and POI distributions near Liangmaqiao Station, Beijing: 1)~there're a lot of restaurants, hotels, and ambassies near the station. This leads to a high flow rate of both working and entertaining, and thus a big demand for vehicle parkings. 2)~The roads around ambassies get high ranks. 3)~The lanes along with Dongsanhuan roads have good condition in overall.
%    When we arrive at Liangmaqiao station, we discover that 1)~Around the ambassy region, the parking lots are poorly built. As a consequence, people working and have meals nearby have to leave their cars in non-parking area, blocking the bike lanes or even zebra crossing, as is shown in Figure~\ref{fig:exp:case}b. Note that all the cars within the figure are parking. 2)~Along with Dongsanhuan road, the POI is relatively sparse, especially in the east side, there are two big hotels and Agriculture Exhibition Center, with large parking lots inside. Therefore, the road is clean with few parking issues (Figure~\ref{fig:exp:case}c).
\begin{figure}[t]
  \begin{center}
  \includegraphics[width=3.5in]{./Figures/overallcase.pdf}      
    \caption{Case Study of Overall Ranking.}
  \label{fig:exp:overallcase}
  \end{center}
  \vspace{-20pt}
\end{figure}
  
\sstitle{Impact of Rush Hours} The KS statistic varies differently at different times on a road segment, which indicates the the temporal differences of illegal parking events. We studied a road segment near Liangmaqiao Subway station, whose KS statistic is significantly higher during the rush hour, as shown in Figure~\ref{fig:exp:temporalcases}a. We visit the area multiple times and notice that, during the evening rush hours, we notice much more illegal parking events: either from some uber/didi drivers waiting for their customers from the subway station, or some people who visit the nearby restaurants and didn't find a parking space.

% where illegal parking issues are more likely to happen during rush hours. Figure~\ref{fig:exp:case}f presents a road near Liangmaqiao Station which is detected to have illegal parkings during night rush hours. When we arrive there, we discovered that this road is near from the subway export, and as is shown Figure~\ref{fig:exp:case}g, there is no illegal parking during work hours, while there are cars during the night rush hours. This can be interpreted that, during the night rush hours,

\sstitle{Impact of Holiday Events} It is also interesting to observe that a local park (Wanghe Park) near Wangjing area, is significantly impacted by different days. We notice that the road in Figure~\ref{fig:exp:temporalcases}b has significantly different KS statistics at the same time between weekdays and weekends. After we got there, we notice that the park is holding a snow festival. A lot of children practice skiing there, as the PyeongChang Winter Olympic Games is approaching. As a result, there are much more illegal curbside vehicle parking events during the weekends, as some of the parents can not find a parking space nearby.
%
%We further studied the time of the illegal parkings' occurrence, and find two interesting patterns: 1)~Sensitive to holiday. We notice that the roads in the north-east of Taiyanggong Park (Figure~\ref{fig:exp:case}d) had illegal parking issues during Chinese YuanDan holiday. This is because, there was a big entertainment activity, causing a lot of people fleed in. As a result, as is shown in Figure~\ref{fig:exp:case}e, many cars were parked, but in contrast, there are merely no cars during workdays.
%    
%    It should be noted that the roads sensitive to rush hours or holidays may get low ranks. E.g. the road in Figure~\ref{fig:exp:case}f belongs to the lowest rank in Figure~\ref{fig:exp:case}a.






==> future.tex <==
\section{Future Work}\label{sec:future}


\begin{figure}[b]
  \vspace{-15pt}
  \begin{center}
    \includegraphics[width=3.4in]{./Figures/future.pdf}
    \caption{Future Work.}
  \label{fig:future}
  \end{center}
\end{figure}

In this paper, we focus on the illegal parkings happening at curbsides, and propose a data-driven illegal parking detection framework based on the data mining results from massive sharing bike trajectories. However, just using the bike trajectories is not the silver bullet to solve the illegal parking detection. In the future, we plan to extend the work to address the following two problems: 1)~distinguishing illegal parkings from other events that influence the bike trajectories. Figure~\ref{fig:future}a gives an example of road maintaining, where the riders are forced to vehicle lanes, which leads the changes in trajectory patterns. Also, some of the curbsides can provide legal parking space; and 2)~detecting the illegal parkings out of curbsides. As is shown in Figure~\ref{fig:future}b, the parked cars blocks the partial of the vehicle lanes. However, they do not affect to the passing-by bike trajectories, which may lead to false negative result in our settings. 



